Mind the Tail: Data Selection Through Sparse Concepts

Data selection reallocates training support across visual concepts, including objects, attributes, color, texture, and backgrounds. Different allocation strategies may produce varied downstream model behavior, especially for tail concepts supported by only a few samples. Discarding them can hurt test-time robustness, while overemphasizing samples lying on category boundaries may introduce unstable training signals. This work explicitly investigates this relationship across fine-grained, spurious-correlation, and general image classification, as well as multimodal pretraining. Specifically, we use sparse autoencoders (SAEs) to extract concept activations from individual images. During selection, we accumulate the dataset-level concept support for each added sample. Applying diminishing returns to this distribution down-weights well-represented concepts and shifts the focus to the distribution tail. We then incorporate local support to find samples that reliably strengthen under-supported concepts. Empirical results show consistent improvements over strong data selection baselines across all benchmarks. We also reveal the connection between concepts our method enhances and the induced behavioral changes, including improved robustness against out-of-distribution and spurious contexts. This work establishes concept support, beyond individual sample importance, as a useful principle for data-efficient and robust learning.

==> tables/abl_beta_main.tex <==
\captionof{table}{\textbf{Sensitivity to the neighborhood weight $\beta$.}
We vary the neighborhood weight $\beta$ and evaluate its effect across
general, fine-grained, and spurious classification settings.}
\label{tab:abl_beta}

\vspace{3pt}

\begingroup
\small
\setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.08}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}c ccc ccc ccc@{}}
\toprule
\multirow{2}{*}{$\boldsymbol{\beta}$}
& \multicolumn{3}{c}{\textbf{General}}
& \multicolumn{3}{c}{\textbf{Fine-grained}}
& \multicolumn{3}{c}{\textbf{Spurious}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}

& 10\% & 30\% & 50\%
& 10\% & 30\% & 50\%
& 10\% & 30\% & 50\% \\

\midrule

$0$
& $12.0$ & $32.5$ & $45.1$
& $37.9$ & $66.6$ & $75.0$
& $65.7$ & $75.9$ & $79.1$ \\

$0.05$
& $15.4$ & $37.0$ & $46.5$
& $42.9$ & $67.4$ & $75.2$
& $68.6$ & $77.9$ & $79.3$ \\

$0.1$
& $15.7$ & $36.9$ & $46.6$
& $42.8$ & $67.2$ & $75.0$
& $66.6$ & $71.7$ & $78.4$ \\

$0.25$
& $16.8$ & $34.7$ & $45.1$
& $42.7$ & $67.3$ & $74.5$
& $65.7$ & $76.5$ & $79.3$ \\

$0.5$
& $21.1$ & $38.3$ & $45.9$
& $42.6$ & $67.0$ & $74.1$
& $69.8$ & $75.4$ & $75.9$ \\

$1.0$
& $22.3$ & $39.2$ & $48.7$
& $42.3$ & $66.1$ & $73.7$
& $65.4$ & $75.4$ & $74.8$ \\

$2.0$
& $\mathbf{23.5}$ & $\mathbf{40.4}$ & $\mathbf{50.0}$
& $41.9$ & $66.0$ & $73.3$
& $65.4$ & $67.6$ & $77.3$ \\

\bottomrule
\end{tabular}
}
\endgroup

==> tables/abl_overview_k_and_activation.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}[t]{0.47\textwidth}
\vspace{0pt}
\centering
\input{tables/abl_k}
\end{minipage}
\hfill
\begin{minipage}[t]{0.51\textwidth}
\vspace{0pt}
\centering
\input{tables/abl_activation_function}
\end{minipage}

\end{figure*}

==> tables/abl_pretrain_feature.tex <==
\captionof{table}{\textbf{Robustness to different pretrained features} used for SAE training and subset selection.
The best and second-best results in each column are bolded and underlined, respectively.}
\label{tab:feature_robustness}

\vspace{-4pt}

\begingroup
\small
\setlength{\tabcolsep}{3.0pt}
% \renewcommand{\arraystretch}{1.08}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}l ccc ccc@{}}
\toprule
\multirow{2}{*}{\makecell[l]{\textbf{Pretrained} \\\textbf{Feature}}}
& \multicolumn{3}{c}{\textbf{NABirds Acc}}
& \multicolumn{3}{c}{\textbf{Waterbirds WGA}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& 10\% & 30\% & 50\%
& 10\% & 30\% & 50\% \\
\midrule

DINOv2-B
& $42.7$ & $\mathbf{68.1}$ & $\mathbf{75.3}$
& $70.1$ & $76.0$ & $79.2$ \\

DINOv3-S
& $\mathbf{43.2}$ & $\underline{67.5}$ & $\mathbf{75.3}$
& $\mathbf{71.5}$ & $\mathbf{79.4}$ & $79.5$ \\

DINOv3-B
& $\underline{42.9}$ & $67.4$ & $\underline{75.2}$
& $68.6$ & $\underline{77.9}$ & $79.3$ \\

CLIP ViT-B/16
& $\underline{42.9}$ & $67.0$ & $74.9$
& $69.6$ & $77.6$ & $\mathbf{80.8}$ \\

SigLIP 2
& $40.3$ & $67.2$ & $74.9$
& $\underline{70.7}$ & $76.6$ & $\underline{79.9}$ \\

\bottomrule
\end{tabular}
}
\endgroup
